Discovering COVID-19 Coughing and Breathing Patterns from Unlabeled Data Using Contrastive Learning with Varying Pre-Training Domains

Rapid discovery of new diseases, such as COVID-19 can enable a timely epidemic response, preventing the large-scale spread and protecting public health. However, limited research efforts have been taken on this problem. In this paper, we propose a contrastive learning-based modeling approach for COVID-19 coughing and breathing pattern discovery from non-COVID coughs. To validate our models, extensive experiments have been conducted using four large audio datasets and one image dataset. We further explore the effects of different factors, such as domain relevance and augmentation order on the pre-trained models. Our results show that the proposed model can effectively distinguish COVID-19 coughing and breathing from unlabeled data and labeled non-COVID coughs with an accuracy of up to 0.81 and 0.86, respectively. Findings from this work will guide future research to detect an outbreak of a new disease early.

==> old-approach.tex <==
\section{Approach}\label{approach}

\subsection{Datasets}
\subsection{Data Processing}
\subsection{Methods}

\textcolor{blue}{to be added, the cough phase}


Cough audio samples from COSWARA, FluSense, ESC-50 and AudioSet are recordings contains multiple individual cough events, so we firstly process the raw recordings into separate clips so that each clip only contains one cough event. Left boxplot of Fig.\ref{0.5s} shows the distribution of the duration of all cough samples after processing. We then choose 0.5s as the uniform time window for all input data because more than 75\% of samples lie under this threshold for each dataset. After dumping out out-of-distribution samples, we use zero-padding to make up for the difference for samples which durations are less than 0.5s, and intercept central 0.5s clips for samples which durations are more than 0.5s. 
\begin{figure}[t]
\centering
\includegraphics[width=3.0in]{fig/20230217.pdf}
\caption{Distribution of duration of the segmented coughing samples and mean value of pixels of Log-Mel spectrograms of all processed samples.}
\label{0.5s}
\end{figure}


Since the breathing event is continuous, we simply segment all the breathing recordings into 0.5s window size. After processing, there also exists clips that contains very few information because they happen to be at the end or beginning of one breathing cycle. We need to delete those samples for the best performance without disturbance. Right boxplot of Fig.\ref{0.5s} shows the distribution of average pixel values of all Log-Mel spectrograms transformed from breathing samples after segmentation. We choose 70 as the threshold and delete all clips under the threshold. To balance the dataset, the training set of each class is then sampled down to 1600 samples. We do the similar pre-processing to pre-trained datasets, too. At last, there are 380 samples in  each class for ESC-50 and 900 samples in each class for AudioSet that are used for pre-training. 

\begin{figure}[t]
\centering
\includegraphics[width=3.0in]{fig/dg.pdf}
\caption{The illustration of two different data augmentation approaches for pre-trained models.(a) illustrates the Image Augmentation(IA) method while (b) illustrates the Audio Augmentation(AA) method. augmentation ordering combine images}
\label{approachjpg}
\end{figure}
%----------------------------
after all these processing, we end up with x number of sample per class for esc 50 dataset y number of samples z numbers for cough dataset. w number of cifar 
%------------------------------

\subsection{Creating Pre-trained Model}
The pre-trained model is used to extract a general-purpose representation of Log-Mel spectrograms from unlabelled data with a contrastive loss function. First, we transform each sample with two random strategies in the data augmentation module. The augmented samples are then put into the neural network base encoders to extract representation vectors. Here we choose ResNet-50 and remove the final FC layer as the backbone. Following the work of SimCLR\cite{chen2020simple}, the extracted vectors are then put into a small MLP network with one hidden layer that projects the representations into an embedding space where contrastive loss functions are applied to maximize the similarity between correlated samples. After the pre-training, the projection head is abandoned and representations from encoders are used for unknown disease detection tasks.
In this paper, we utilize two different data augmentation strategies for pre-training: 
\subsubsection{Image Augmentation(IA)}
Figure \ref{approachjpg}(a) shows our first augmentation strategy: Image Augmentation(IA). The audio clips from samples are firstly transformed to Log-Mel spectrograms, then they are applied two random image augmentation methods: (1) Random Cropping, a random area from the Log-Mel spectrogram is cropped followed by resize original size;(2) Gaussian Blur: a method of data smoothing.
\subsubsection{Audio Augmentation(AA)}
Figure \ref{approachjpg}(b)shows our second augmentation strategy: Audio Augmentation(IA). The audio clips from samples are firstly augmented by open source WavAug tool with random pitch shift and room reverberation first, then they are transformed to Log-Mel spectrograms.
\subsection{Model Framework}
\textcolor{blue}{open world contrastive learning framework }




==> old-data_collection.tex <==
\section{Data Collection}\label{datacollection}
In this section, we will discuss datasets that we use for pre-training as well as unknown disease detection model. 


\subsection{Pre-training Dataset}
We use three different datasets for pre-training: CIFAR10, ESC-50 and AudioSet. 
CIFAR-10 is a commonly used benchmark for object classification. It consists of 60,000 color images in 10 classes, with 6,000 images per class. 
%/full name event
%--------------------------------------
%/categoty by dataset

ESC-50 are widely-used audio datasets with 50 classes of acoustic events, with 40 recordings of 5 seconds per class. In our experiments, cough and breathing classes are excluded to ensure the model doesn't have bias towards cough or breathing sound. Therefore, there are 48 classes from ESC-50 dataset that are used for pre-training. 
AudioSet is a large-scaled acoustic datasets which contains 632 kinds of sounds extracted from Youtube videos, with over 2 million human-labelled 10 second audio clips. In our experiment, the subset of human sounds from AudioSet is used which only contains 48 classes sounds that are generated from human mouths and noses, such as snoring, sneezing, singing and crying, without cough and breathing.

\subsection{Cough and Breathing Dataset}
We make our dataset with four classes from COSWARA, FluSense, ESC-50 and AudioSet. COSWARA is a project proposed by Indian Institute of Science (IISc) Bangalore which contributes to build a large COVID-19 dataset of audio recordings such as breathing, cough and speech sounds from COVID-19 positive and non-COVID-19 individuals. FluSense is a large-scaled multi-sound dataset recorded in four public waiting areas within the hospital of a large university to track influenza-related indicators. 

In our experiment settings, the four classes are: healthy people coughing(Healthy), flu patient coughing(Flu), COVID-19 patient coughing(CC), and COVID-19 patient breathing(CB). Among them, healthy people cough sounds are collected from COSWARA non-COVID-19 subjects, ESC-50 and AudioSet. Flu patients' coughing are collected from FluSense Dataset, COVID-19 patients' coughing and breathing sound are selected from COSWARA positive patients' data.

Furthermore, samples from same subject are kept only in training or test to avoid possible false prediction due to overfitting. The ratio of training set and test set samples is 0.8:0.2.

==> old-evaluation.tex <==
\section{Evaluation}\label{evaluation}
In this section, we provide details of our experiments' settings as well as comparisons between different settings.
\subsection{Experiment Settings}
Our study aimed to investigate the potential effects of using different contrastive learning pre-trained models on the performance of unknown disease detection. To this end, we acquired multiple pre-trained models with different settings and datasets. 

To closely replicate real-world scenarios, we assumed that new unknown disease samples can arise along with existing known disease samples in natural settings. Unknown disease classes were unlabeled, and some known disease classes were also unlabeled. In our experiments, we treated COVID-19 coughing (CC) and COVID-19 breathing (CB) as unknown classes without any labels during the training process. Known classes were healthy coughing and flu coughing, of which 90\% of the samples were labeled, and 10\% were unlabeled.

To reduce randomness, we trained each disease detection model five times for each pre-trained model, and randomly partitioned the test sets into ten subsets. For each unknown detection model, we performed ten tests on the subsets. Therefore, we analyzed fifty results for each pre-trained model.

%To eliminate randomness, for each pre-trained model, we did disease detection model training for five times. Test sets are randomly segmented into 10 subsets. For each unknown detection model, 10 subsets were tested. Therefore, in analyzing each pre-trained model, 50 results were considered

\subsection{Performance of Different Pre-trained Models}\label{}

%\subsubsection{Effects of Dataset Types}
\subsubsection{Effects of Dataset Types}
Fig.\ref{cifar-esc50}

\begin{figure}[t]
\centering
\includegraphics[width=3.0in]{fig/cifar10.png}
\caption{Unknown disease detection performance using pre-trained models trained on different types of datasets.}
\label{cifar-esc50}
\end{figure}

\subsubsection{Effects of Dataset Relevance}
Fig.\ref{human-non-human}
\begin{figure}[t]
\centering
\includegraphics[width=3.0in]{fig/human.png}
\caption{Unknown disease detection performance using pre-trained models trained on subsets from ESC-50 with different levels of relevance to human sounds. }
\label{human-non-human}
\end{figure}

\subsubsection{Effects of Dataset Size}
Fig.
%\begin{figure}[t]
%\centering
%\includegraphics[width=3.0in]{fig/figure_name}
%\caption{}
%\label{human-non-human}
%\end{figure}

\subsection{Performance of Different Augmentation Methods}
Fig.\ref{all}
\begin{figure}[t]
\centering
\includegraphics[width=3.0in]{fig/all.png}
\caption{}
\label{all}
\end{figure}

